Parsimonious inertial cavitation rheometry via bubble collapse time

The rapid and accurate characterization of soft, viscoelastic materials at high strain rates is of interest in biological and engineering applications. Examples include assessing the extent of tissue ablation during histotripsy procedures and developing injury criteria for the mitigation of blast injuries. The inertial microcavitation rheometry technique (IMR, Estrada et al., 2018) allows for the characterization of local viscoelastic properties at strain rates up to 1E8 per second. However, IMR now typically relies on bright-field videography of a sufficiently translucent sample at >1 million frames per second and a simulation-dependent fit optimization process that can require hours of post-processing. Here, we present an improved IMR-style technique, called parsimonious inertial microcavitation rheometry (pIMR), that parsimoniously characterizes surrounding viscoelastic materials. The pIMR approach uses experimental advancements to estimate the time to first collapse of the laser-induced cavity within approximately 20 ns and a theoretical energy balance analysis that yields an approximate collapse time based on the material viscoelasticity parameters. The pIMR method closely matches the accuracy of the original IMR procedure while decreasing the computational cost from hours to seconds while potentially reducing reliance on ultra-high-speed videography. This technique can enable nearly real-time characterization of soft, viscoelastic hydrogels and biological materials with a numerical criterion assessing the correct choice of model. We illustrate the efficacy of the technique on batches of tens of experiments for both soft hydrogels and fluids.

==> newcommands_all.tex <==
% This file is not actually included. Paste commands here for reference.

%% Self-defined Macros
\newcommand{\bn}[1]{\mathbf{#1}}
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\norm}[1]{\ensuremath \lVert #1 \rVert}
\newcommand{\GD}[1]{ D #1 (\boldsymbol{F})[\boldsymbol{H}]}
\newcommand{\GDI}[1]{ D #1 (\boldsymbol{I})[\boldsymbol{H}]}
\newcommand{\Lin}[1]{ L_{\boldsymbol{F}} #1 [\boldsymbol{H}]}
\newcommand{\LinI}[1]{ L_{\boldsymbol{I}} #1 [\boldsymbol{H}]}
\newcommand{\Dm}[1]{\ensuremath{\boldsymbol{\varphi} } }
\newcommand{\tr}[1]{\textcolor{red}{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\fracp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\wt}[1]{\widetilde{#1}}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\newcommand{\tn}{\textnormal}

%% Coloring for comments
\usepackage{color,tikz,soul}
\newcommand{\jbe}[1]{\textcolor{violet}{#1}}
\newcommand{\zz}[1]{\textcolor{teal}{#1}}
\newcommand{\ba}[1]{\textcolor{brown}{#1}}
\newcommand{\sr}[1]{\textcolor{magenta}{#1}}
\newcommand{\atjbe}[1]{\textcolor{blue}{\textbf{@JBE:} #1}}
\newcommand{\atzz}[1]{\textcolor{green}{\textbf{@ZZ:} #1}}
\newcommand{\atba}[1]{\textcolor{orange}{\textbf{@BA:} #1}}
\newcommand{\atsr}[1]{\textcolor{purple}{\textbf{@SR:} #1}}



\usepackage{xcolor, soul}
\sethlcolor{yellow}
\usepackage[per-mode=symbol]{siunitx}

\setlength{\tabcolsep}{12pt}

\renewcommand{\thetable}{\arabic{table}} % Originally Roman uppercase





 %% Below are old commands from the MR-u paper. Commented but kept for reference.
 
% \definecolor{lightblue}{rgb}{0, 0.5, 1}
% \definecolor{gray}{rgb}{0.6, 0.6, 0.6}
% \definecolor{dkred}{rgb}{0.5, 0, 0}
% \definecolor{dkblue}{rgb}{0, 0, 0.5}
% \definecolor{dkgreen}{rgb}{0, 0.5, 0}
% \definecolor{dkteal}{rgb}{0, 0.5, 0.5}

% \newcommand{\bn}[1]{\mathbf{#1}}
% %\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}
% %\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
% %\newcommand{\norm}[1]{\ensuremath \lVert #1 \rVert}
% %\newcommand{\GD}[1]{ D #1 (\boldsymbol{F})[\boldsymbol{H}]}
% %\newcommand{\GDI}[1]{ D #1 (\boldsymbol{I})[\boldsymbol{H}]}
% %\newcommand{\Lin}[1]{ L_{\boldsymbol{F}} #1 [\boldsymbol{H}]}
% %\newcommand{\LinI}[1]{ L_{\boldsymbol{I}} #1 [\boldsymbol{H}]}
% %\newcommand{\Dm}[1]{\ensuremath{\boldsymbol{\varphi} } }
% \newcommand{\instr}[1]{\textcolor{gray}{#1}}
% \newcommand{\ums}[1]{\textcolor{dkblue}{#1}}
% \newcommand{\cml}[1]{\textcolor{dkgreen}{#1}}
% \newcommand{\jbe}[1]{\textcolor{dkteal}{#1}}
% \newcommand{\ema}[1]{\textcolor{dkred}{#1}}
% \newcommand{\CITE}[1]{\textcolor{red}{\textbf{[CITE:} #1\textbf{]}}}
% \newcommand{\REF}[1]{\textcolor{blue}{\textbf{[REF:} #1\textbf{]}}}
% \newcommand{\COMPANY}[1]{\textcolor{green}{\textbf{[Company:} #1\textbf{]}}}
% \newcommand{\ignore}[1]{}
% %\newcommand{\fracp}[2]{\frac{\partial #1}{\partial #2}}
% \newcommand{\wt}[1]{\widetilde{#1}}
% \usepackage{bm}
% %\newcommand{\fracptwo}[2]{\frac{\partial ^2 #1}{\partial #2 ^2}}



% \newcommand{\lls}{l1\underline{\hspace{0.5em}}ls}
% \newcommand{\sparsa}{SpaRSA}
% \newcommand{\cgist}{CGIST}
% \newcommand{\fpcas}{FPC\underline{\hspace{0.5em}}AS}
% \newcommand{\admm}{ADMM}

% \renewcommand{\arraystretch}{1.2}

% % Common formatting.
% \renewcommand{\[}{\left[}
% \renewcommand{\]}{\right]}
% \renewcommand{\(}{\left(}
% \renewcommand{\)}{\right)}

% % Common operators.
% \newcommand{\dd}[2]{\frac{d #1}{d #2}}
% \newcommand{\ddt}[1]{\frac{d #1}{d t}}
% \newcommand{\ddd}[2]{\frac{d^2 #1}{d #2^2}}
% \newcommand{\dddt}[1]{\frac{d^2 #1}{d t^2}}
% \newcommand{\pp}[2]{\frac{\partial #1}{\partial #2}}
% \newcommand{\ppp}[2]{\frac{\partial^2 #1}{\partial #2^2}}
% \newcommand{\pppp}[2]{\frac{\partial^3 #1}{\partial #2^3}}
% \newcommand{\ppppp}[2]{\frac{\partial^4 #1}{\partial #2^4}}

% \newcommand{\adj}[1]{#1^{*}}
% \newcommand{\abs}[1]{\left|#1\right|}
% \newcommand{\divergence}[1]{\nabla \cdot #1}
% \newcommand{\enorm}[1]{\vvvert #1 \vvvert}
% \newcommand{\grad}[1]{\nabla #1}
% \newcommand{\bgrad}[1]{\mathbf{\nabla} #1}
% \newcommand{\laplace}[1]{\nabla^2 #1}
% \newcommand{\norm}[2]{\left\|\, #1 \,\right\|_{#2}}
% \newcommand{\order}[1]{\mathcal{O}\(#1\)}
% \newcommand{\supp}{\mathop{\mathrm{supp}}}
% %\newcommand{\vvvert}{|\kern-1pt|\kern-1pt|}

% \newcommand{\eq}[1]{\mathop{\,{\buildrel #1 \over =}\,}}
% \newcommand{\ap}[1]{\mathop{\,{\buildrel #1 \over \approx}\,}}

% % Modified/combined symbols.

% % Hats.
% \newcommand{\hg}{\hat{g}}
% \newcommand{\hh}{\hat{h}}
% \newcommand{\hi}{\hat{i}}
% \newcommand{\hj}{\hat{j}}
% \newcommand{\hk}{\hat{k}}
% %\newcommand{\hm}{\hat{m}}
% \newcommand{\hn}{\hat{n}}
% \newcommand{\hs}{\hat{s}}
% \newcommand{\hu}{\hat{u}}
% \newcommand{\hv}{\hat{v}}
% \newcommand{\hx}{\hat{x}}

% \newcommand{\hA}{\hat{A}}
% \newcommand{\hC}{\hat{C}}
% \newcommand{\hI}{\hat{I}}
% \newcommand{\hJ}{\hat{J}}
% \newcommand{\hN}{\hat{N}}
% \newcommand{\hT}{\hat{T}}
% \newcommand{\hU}{\hat{U}}

% \newcommand{\hbf}{\boldsymbol{\hat{f}}}
% \newcommand{\hbg}{\boldsymbol{\hat{g}}}
% \newcommand{\hsig}{\hat{\sigma}}

% % Bar.
% \newcommand{\barg}{\bar{g}}
% \newcommand{\barh}{\bar{h}}
% \newcommand{\barm}{\bar{m}}
% \newcommand{\barv}{\bar{v}}
% \newcommand{\barw}{\bar{w}}
% \newcommand{\barx}{\bar{x}}
% \newcommand{\bary}{\bar{y}}

% \newcommand{\barB}{\bar{B}}
% \newcommand{\barC}{\bar{C}}
% \newcommand{\barH}{\bar{H}}
% \newcommand{\barJ}{\bar{J}}
% \newcommand{\barN}{\bar{N}}
% \newcommand{\barR}{\bar{R}}

% \newcommand{\barmu}{\bar{\mu}}

% % Tilde.
% \newcommand{\tf}{\tilde{f}}
% \newcommand{\thh}{\tilde{h}}

% \newcommand{\tA}{\tilde{A}}
% \newcommand{\tg}{\tilde{g}}
% \newcommand{\tH}{\tilde{H}}
% \newcommand{\tJ}{\tilde{J}}
% \newcommand{\tQ}{\tilde{Q}}
% \newcommand{\tT}{\tilde{T}}

% \newcommand{\tmu}{\tilde{\mu}}
% \newcommand{\ttheta}{\tilde{\theta}}
% \newcommand{\txi}{\tilde{\xi}}

% \newcommand{\tTheta}{\tilde{\Theta}}
% \newcommand{\tXi}{\tilde{\Xi}}

% \newcommand{\td}{\tilde{d}}

% % Bold.
% \newcommand{\mb}[1]{\mathbf{#1}}
% \newcommand{\sbf}[1]{\boldsymbol{#1}}

% \newcommand{\ba}{\textbf{a}}
% \newcommand{\bb}{\textbf{b}}
% \newcommand{\bd}{\textbf{d}}
% \newcommand{\bee}{\textbf{e}}
% \newcommand{\bff}{\textbf{f}}
% \newcommand{\bh}{\textbf{h}}
% \newcommand{\bg}{\textbf{g}}
% \newcommand{\bk}{\textbf{k}}
% \newcommand{\bii}{\textbf{i}}
% \newcommand{\bj}{\textbf{j}}
% \newcommand{\bl}{\textbf{l}}
% \newcommand{\bnn}{\textbf{n}}
% \newcommand{\bp}{\textbf{p}}
% \newcommand{\br}{\textbf{r}}
% \newcommand{\bs}{\textbf{s}}
% \newcommand{\bt}{\textbf{t}}
% \newcommand{\bu}{\textbf{u}}
% \newcommand{\bv}{\textbf{v}}
% \newcommand{\bw}{\textbf{w}}
% \newcommand{\bx}{\textbf{x}}
% \newcommand{\by}{\textbf{y}}

% \newcommand{\bA}{\mathbf{A}}
% \newcommand{\bC}{\mathbf{C}}
% \newcommand{\bE}{\mathbf{E}}
% \newcommand{\bF}{\mathbf{F}}
% \newcommand{\bG}{\mathbf{G}}
% \newcommand{\bI}{\mathbf{I}}
% \newcommand{\bK}{\mathbf{K}}
% \newcommand{\bN}{\mathbf{N}}
% \newcommand{\bP}{\mathbf{P}}
% \newcommand{\bQ}{\mathbf{Q}}
% \newcommand{\bR}{\mathbf{R}}
% \newcommand{\bT}{\mathbf{T}}
% \newcommand{\bU}{\mathbf{U}}
% \newcommand{\bV}{\mathbf{V}}
% \newcommand{\bX}{\mathbf{X}}
% \newcommand{\bY}{\mathbf{Y}}

% \newcommand{\balpha}{\boldsymbol{\alpha}}
% \newcommand{\bbeta}{\boldsymbol{\beta}}
% \newcommand{\bepsilon}{\boldsymbol{\epsilon}}
% \newcommand{\bhsig}{\boldsymbol{\hsig}}
% \newcommand{\bpsi}{\boldsymbol{\psi}}
% \newcommand{\bsig}{\boldsymbol{\sigma}}
% \newcommand{\btau}{\boldsymbol{\tau}}
% \newcommand{\bmu}{\boldsymbol{\mu}}
% \newcommand{\bpi}{\boldsymbol{\pi}}
% \newcommand{\btheta}{\boldsymbol{\theta}}
% \newcommand{\bphi}{\boldsymbol{\phi}}
% \newcommand{\bxi}{\boldsymbol{\xi}}
% \newcommand{\bchi}{\boldsymbol{\chi}}

% \newcommand{\bDelta}{\boldsymbol{\Delta}}
% \newcommand{\bTheta}{\boldsymbol{\Theta}}
% \newcommand{\bXi}{\boldsymbol{\Xi}}
% \newcommand{\bPi}{\boldsymbol{\Pi}}
% \newcommand{\bOmega}{\boldsymbol{\Omega}}
% \newcommand{\bSigma}{\boldsymbol{\Sigma}}

% % Shadow.
% \newcommand{\EE}{\mathbb{E}}
% \newcommand{\II}{\mathbb{I}}
% \newcommand{\NN}{\mathbb{N}}
% \newcommand{\QQ}{\mathbb{Q}}
% \newcommand{\PP}{\mathbb{P}}
% \newcommand{\RR}{\mathbb{R}}

% % Vec.
% \newcommand{\vt}{\vec{t}}
% \newcommand{\vu}{\vec{u}}
% \newcommand{\vv}{\vec{v}}
% \newcommand{\vx}{\vec{x}}

% \newcommand{\vV}{\vec{V}}

% \newcommand{\vo}{\vec{\omega}}

% % Dot.
% \newcommand{\dotk}{\dot{k}}
% \newcommand{\dotm}{\dot{m}}
% \newcommand{\dotx}{\dot{x}}

% \newcommand{\dotomega}{\dot{\omega}}

% % Mathcal.
% \newcommand{\CA}{\mathcal{A}}
% \newcommand{\CB}{\mathcal{B}}
% \newcommand{\CD}{\mathcal{D}}
% \newcommand{\CE}{\mathcal{E}}
% \newcommand{\CF}{\mathcal{F}}
% \newcommand{\CH}{\mathcal{H}}
% \newcommand{\CJ}{\mathcal{J}}
% \newcommand{\CK}{\mathcal{K}}
% \newcommand{\CL}{\mathcal{L}}
% \newcommand{\CM}{\mathcal{M}}
% \newcommand{\CN}{\mathcal{N}}
% \newcommand{\CR}{\mathcal{R}}
% \newcommand{\CS}{\mathcal{S}}
% \newcommand{\CT}{\mathcal{T}}
% \newcommand{\CU}{\mathcal{U}}
% \newcommand{\CV}{\mathcal{V}}
% \newcommand{\CW}{\mathcal{W}}
% \newcommand{\CX}{\mathcal{X}}
% \newcommand{\CY}{\mathcal{Y}}

% \newcommand{\CbarJ}{\bar{\mathcal{J}}}
% \newcommand{\CbarL}{\bar{\mathcal{L}}}
% \newcommand{\CbarR}{\bar{\mathcal{R}}}

% % Delta.
% \newcommand{\du}{\delta{u}}

% \newcommand{\dbeta}{\delta{\beta}}
% \newcommand{\dxi}{\delta{\xi}}
% \newcommand{\deta}{\delta{\eta}}
% \newcommand{\drho}{\delta{\rho}}
% \newcommand{\dtau}{\delta{\tau}}

% \newcommand{\dbu}{\delta{\boldsymbol{u}}}
% \newcommand{\dbp}{\delta{\boldsymbol{p}}}
% \newcommand{\dbx}{\delta{\boldsymbol{x}}}

% \newcommand{\Dx}{\Delta{x}}
% \newcommand{\Dy}{\Delta{y}}
% \newcommand{\Dt}{\Delta{t}}

% % Colors.
% % \newcommand{\myblue}[1]{{\color[rgb]{0,0,0.65} #1}}
% % \newcommand{\mygreen}[1]{{\color[rgb]{0,.65,0} #1}}
% % \newcommand{\mywhite}[1]{{\color[rgb]{1.0,1.0,1.0} #1}}
% % \newcommand{\myred}[1]{{\color[rgb]{0.65,0.0,0.0} #1}}
% % \newcommand{\myblack}[1]{{\color[rgb]{0.0,0.0,0.0} #1}}
% % \newcommand{\mygrey}[1]{{\color[rgb]{0.6,0.6,0.6} #1}}

% % Chemicals.
% \newcommand{\coo}{CO$_2$}
% \newcommand{\hho}{H$_2$O}
% \newcommand{\oo}{O$_2$}
% \newcommand{\nn}{N$_2$}
% \newcommand{\mwe}{MW$_e$}
% \newcommand{\nox}{NO$_{\textrm{x}}$}
% \newcommand{\cooe}{CO$_{2e}$}
% \newcommand{\nno}{N$_2$O}
% \newcommand{\noo}{NO$_2$ }
% \newcommand{\chhhh}{CH$_4$ }
% \newcommand{\hhoo}{H$_2$O$_2$}
% \newcommand{\hhoor}{H$_2$-O$_2$}

% % Units.
% \newcommand{\degs}{^\circ}
% \newcommand{\Jpkmol}{\frac{J}{kmol}}
% \newcommand{\JpkmolK}{\frac{J}{kmol K}}
% \newcommand{\Jpkg}{\frac{J}{kg}}
% \newcommand{\JpkgK}{\frac{J}{kg K}}
% \newcommand{\rmu}{$\upmu$}

% % Others.
% \newcommand{\ra}{\rightarrow}
% \newcommand{\Ra}{\Rightarrow}
% \newcommand{\LRa}{\Longrightarrow}
% \newcommand{\lra}{\longrightarrow}

% \newcommand{\pe}{\,{\scriptstyle +}\!\!=}
% \newcommand{\me}{\,{\scriptstyle -}\!\!=}
% \newcommand{\Var}{\textrm{Var}}
% \newcommand{\Cov}{\textrm{Cov}}
% \newcommand{\diag}{\textrm{diag}}

% \newcommand{\etal}{\textit{et al.}}

% \def\sgn{\mathop{\rm sgn}}
% \newcommand{\argmax}{\operatornamewithlimits{argmax}}
% \newcommand{\argmin}{\operatornamewithlimits{argmin}}
% \newcommand{\DKL}{D_{\mathrm{KL}}}

% \newcommand{\iid}{\stackrel{\textrm{iid}}{\sim}}
% \newcommand{\ti}[1]{\textbf{Title: }\textit{{#1}}}

% % Theorem styles.
% % \newtheorem{cond}{Condition}[section]

% % \theoremstyle{definition}
% % \newtheorem{definition}{Definition}[section]

% % \theoremstyle{definition}
% % \newtheorem{algo}{Algorithm}[section]

% % \theoremstyle{definition}
% % \newtheorem{example}{Example}[section]

% % % Per SIAM Style Manual, "section" should be lowercase
% % \crefname{section}{section}{sections}
% % \crefname{subsection}{subsection}{subsections}

% % % Per SIAM Style Manual, "Figure" should be spelled out in references
% % \Crefname{figure}{Figure}{Figures}

% % % Per SIAM Style Manual, don't say equation in front on an equation.
% % \crefformat{equation}{\textup{#2(#1)#3}}
% % \crefrangeformat{equation}{\textup{#3(#1)#4--#5(#2)#6}}
% % \crefmultiformat{equation}{\textup{#2(#1)#3}}{ and \textup{#2(#1)#3}}
% % {, \textup{#2(#1)#3}}{, and \textup{#2(#1)#3}}
% % \crefrangemultiformat{equation}{\textup{#3(#1)#4--#5(#2)#6}}%
% % { and \textup{#3(#1)#4--#5(#2)#6}}{, \textup{#3(#1)#4--#5(#2)#6}}{, and \textup{#3(#1)#4--#5(#2)#6}}

% % % But spell it out at the beginning of a sentence.
% % \Crefformat{equation}{#2Equation~\textup{(#1)}#3}
% % \Crefrangeformat{equation}{Equations~\textup{#3(#1)#4--#5(#2)#6}}
% % \Crefmultiformat{equation}{Equations~\textup{#2(#1)#3}}{ and \textup{#2(#1)#3}}
% % {, \textup{#2(#1)#3}}{, and \textup{#2(#1)#3}}
% % \Crefrangemultiformat{equation}{Equations~\textup{#3(#1)#4--#5(#2)#6}}%
% % { and \textup{#3(#1)#4--#5(#2)#6}}{, \textup{#3(#1)#4--#5(#2)#6}}{, and \textup{#3(#1)#4--#5(#2)#6}}

% % % Make number non-italic in any environment.
% % \crefdefaultlabelformat{#2\textup{#1}#3}

